Tunable Luminescence From a Single Free-Base Porphyrin Molecule By Controlled Access to Optically Active States

Scanning tunneling microscopy-induced luminescence (STML) provides access to the optical properties of individual molecules through a cascade of relaxation processes between many-body states. Insufficient charge attachment energies prevent relaxation via optically active states, causing even intrinsically bright molecules to remain dark in STML. Here, we utilize substrate work function control and tip-induced gating of the double-barrier tunnel junction to induce an energy shift of the ionic transition state of a single free-base tetrabenzoporphyrin (H2TBP) to control access to optically active states and bright exciton emission. The experimental observations are validated by a rate equation and a polaron model considering the relaxation energy of the NaCl decoupling layer upon charging of the molecule.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
